TuPAQ: An Efficient Planner for Large-scale Predictive Analytic Queries

The proliferation of massive datasets combined with the development of sophisticated analytical techniques have enabled a wide variety of novel applications such as improved product recommendations, automatic image tagging, and improved speech-driven interfaces. These and many other applications can be supported by Predictive Analytic Queries (PAQs). A major obstacle to supporting PAQs is the challenging and expensive process of identifying and training an appropriate predictive model. Recent efforts aiming to automate this process have focused on single node implementations and have assumed that model training itself is a black box, thus limiting the effectiveness of such approaches on large-scale problems. In this work, we build upon these recent efforts and propose an integrated PAQ planning architecture that combines advanced model search techniques, bandit resource allocation via runtime algorithm introspection, and physical optimization via batching. The result is TuPAQ, a component of the MLbase system, which solves the PAQ planning problem with comparable quality to exhaustive strategies but an order of magnitude more efficiently than the standard baseline approach, and can scale to models trained on terabytes of data across hundreds of machines.

==> architecture.tex <==
\section{Architecture}
\label{sec:architecture}

%\tim{Shouldn't this section be Section 3. This would allow you describe in more detail how you leverage MLI in the optimization Section.}
\mlopt is built on top of Apache Spark and MLI.  These systems have been
designed to support high performance iterative MapReduce algorithms on working
sets that fit into cluster memory, and simplified development of machine
learning algorithms, respectively.  It has been shown that these systems can
outperform conventional MapReduce-based systems for machine learning like
\cite{mahout}, often by an order of magnitude.  We leverage features of both
systems in our design and experiments.  Since both Spark and MLI are written in
Scala, we chose to write \mlopt in Scala as well to  leverage tight integration
with the existing systems and libraries available in the JVM ecosystem.  Our
system is a component of MLbase~\cite{Kraska13},
%- a system under construction that is
%designed to simplify the use of machine learning at scale.
and an important component of MLbase is the MLbase Optimizer, designed to
automate the process of constructing and refining machine learning pipelines.
\mlopt represents a first effort at building such an optimizer and is a central
component to the design of this system.

The architecture of \mlopt consists of three abstract entities: A
\emph{Driver}, one or more \emph{Searchers}, and zero or more \emph{Executors}.
These entities are implemented as \texttt{akka} Actors, which enables a
concurrent programming model that supports asynchronous communication between
these entities.  A graphical depiction of these entities is shown in
Figure~\ref{fig:architecture} and a summary of the protocol between these
entities is captured in Figure~\ref{tab:protocol}.  Additionally, models are trained in a \emph{parallel dataflow} system, whose computational model---iterative MapReduce---lends itself well to expressing a large class of machine
learning algorithms.  The responsibilities of each entity are described below. 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/architecture.pdf}
\caption{The Driver is responsible for defining a search space over which models are to be trained. The Searcher deterimines which configurations to try and, based on the results which ones to try next. It may interact with external search routines to accomplish this. The Executor is responsible for evaluating model configurations and reporting results - it may evaluate a particular configuration over a cluster of machines.}
\label{fig:architecture}
\end{figure}

\subsection{Driver}
The driver is the main entry point for a \mlopt model search. The Driver's
primary responsibilities include instantiating one or more Searchers and
collecting results from the search process.  End users typically interact with
the system through the Driver, which is instantiated with a dataset, a search
space which describes the space of model configurations to explore, and
information about how to configure the searcher and what type of searcher to
instantiate (e.g. Grid, Random, HyperOpt).  The driver communicates asynchronously
with the searcher and collects newly trained models as they become available.
It can also be polled by user programs for new information about search
progress and models that have been trained.

\subsection{Searcher}
A Searcher is responsible for instantiating Executors, deciding on model
configurations for evaluation, farming that work out to its Executors, and
relaying results back to the Driver.  Importantly, we also centralize the
logical and physical optimizations in the implementation of the searcher.
Namely, it is the searcher's job to figure out how best to implement batching
(by sending jobs to a Batch Executor), resource allocation (by evaluating results
from Executors before letting work continue), and to implement the search
method it is responsible for. 

The architecture is such that we may use external libraries or service calls to
implement the searching logic.  For example, in implementing a HyperOpt based
searcher, the HyperOptSearcher code makes external service calls to a web service
that is simply a thin wrapper around the existing Hyperopt
library~\cite{hyperopt}.

By implementing a few concrete methods for suggesting points in the
hyperparameter space and ingesting new results, our system allows easy addition
of new algorithms for hyperparameter optimization as they become available.
Additionally, new algorithms will benefit from the systems level optimizations
made for all algorithms.

\subsection{Executor}
A Executor in \mlopt is an abstract entity capable of evaluating model
configurations.  A \mlopt Executor may launch jobs that are executed on
hundreds of nodes.  In practice, our executors usually have a handle to an
entire cluster, which allows them to execute their jobs in a data parallel
fashion.  As such, we are often in a situation where only a single Executor
needs to be created.  While this detail need not be evident to the searchers, in
the case of batching, for example, the \emph{type} of Executor (that is, a
Batch Executor vs. a Sequential Executor) can play a role in how tasks are
allocated to it.

\begin{figure*}
\begin{tabular}{ll}
\qquad 
\qquad 
\qquad &
  \begin{subtable}[h]{0.30\textwidth}
     \begin{tabular}{|l|l|l|}
			\hline
	    Message                                    & Result     & Meaning                                 \\ \hline
	    RunSearch(space: SearchSpace, data: Table) & ~          & Begin Search Process                    \\ 
	    TopModel()                                 & Model      & Return best model after search.         \\
	    AllBuilt()                                 & Boolean    & Is search process finished?             \\
	    ModelsBuilt()                              & Int        & How many models have been built?        \\
	    Models()                                   & Seq[Model] & Return all models that have been built. \\
			\hline
	    \end{tabular}
			\caption{Driver/Searcher Protocol}
		\end{subtable} \\
& 
		\begin{subtable}[h]{0.30\textwidth}
	    \begin{tabular}{|l|l|l|}
			\hline
	    Message                         & Result  & Meaning                                          \\ \hline
	    BuildModel(config: ModelConfig) & ~       & Add model with this configuration to work queue. \\
	    DoWork()                        & ~       & Begin consuming work queue.                      \\
	    StopWork()                      & ~       & Stop consuming work queue.                       \\
	    QueueSize()                     & Int     & How big is your work queue?                      \\
			\hline
	    \end{tabular}
			\caption{Searcher/Executor Protocol}
		\end{subtable} \\
& 
		\begin{subtable}[h]{0.30\textwidth}
			\begin{tabular}{|l|l|}
					\hline
			    Message                  & Meaning                                                           \\ \hline
			    ModelBuilt(model: Model) & A model has been built with a particular configuration and error. \\ 
			    WorkDone()               & My work queue is empty.                                           \\
					\hline
			    \end{tabular}
		\caption{Executor/Searcher Protocol}
		\end{subtable} \\
  \end{tabular}
  \caption{Summary of protocol between Driver, Searcher, and Executor.} 
		\label{tab:protocol}
\end{figure*}

\subsection{Hybrid Parallel Dataflow and Asynchronous Control for Model Search}
In basing our system on Spark, we are explicitly employing a parallel dataflow
engine to train our models.  At the same time, all of the hyperparameter tuning
happens in an asynchronous fashion with Actors handing out jobs and receiving
results asynchronously.  As such, our system can be viewed as a hybrid of a
traditional BSP computation environment with an asynchronous control plane.  By
employing this approach, we are able to isolate the portions of our system that
need to be high performance, fault tolerant, and data parallel from those that
need to be asynchronous and reactive, leading to a system that achieves both
goals.


==> conclusion.tex <==

In this work, we have demonstrated that by combining better model search methods, batching techniques, and bandit methods for preemptive pruning, we can deliver a system capable of finding high quality query plans for Predictive Analytic Queries on very expensive models trained on very large datasets that is an order of magnitude faster than the baseline approach.
%\mlopt is a component of the MLbase project, and will serve as a foundation for the automated construction of end-to-end pipelines for machine learning.
Moving forward, \mlopt will serve as a foundation for the automated construction of end-to-end pipelines for machine learning.

